On the optimal choice of the illumination function in photoacoustic tomography

This work studies the inverse problem of photoacoustic tomography (more precisely, the acoustic subproblem) as the identification of a space-dependent source parameter. The model consists of a wave equation involving a time-fractional damping term to account for power law frequency dependence of the attenuation, as relevant in ultrasonics. We solve the inverse problem in a Bayesian framework using a Maximum A Posteriori (MAP) estimate, and for this purpose derive an explicit expression for the adjoint operator. On top of this, we consider optimization of the choice of the laser excitation function, which is the time-dependent part of the source in this model, to enhance the reconstruction result. The method employs the $A$-optimality criterion for Bayesian optimal experimental design with Gaussian prior and Gaussian noise. To efficiently approximate the cost functional, we introduce an approximation scheme based on projection onto finite-dimensional subspaces. Finally, we present numerical results that illustrate the theory.

==> numericalresults.tex <==
\section{Numerical results}\label{sec:numerical_results} Finally,  we demonstrate some numerical examples to illustrate our theory.  To begin,  we introduce the general setting that will be used throughout the examples.  For the sake of simplicity, we consider a mathematical example rather than a realistic setup for photoacoustic tomography.  More precisely,  we consider the governing system \eqref{eq:wave_equation} with fixed $c = 300$,  while both $b$ and $\alpha$ might be varied 
%where $b$ depends on $\alpha$.
see Section~\ref{sec:alpha}.
All numerical experiments are performed in a two-dimensional setting with the domain of experiment being $\Omega=[-1,1] \times [-1,1]$ and the observation surface $\Sigma$ being defined by the boundary of $[-0.8,  0.8] \times [-0.8,  0.8]$.  The observation time is $(0,  T)$ with $T = 0.2$.  In order to solve the forward and adjoint problems,  we employ a Newmark time-stepping scheme for fractionally damped wave equations \cite{kaltenbacher_2022} in which the spatial domain is discretized by using the finite element method FEM with $n = 2601$ spatial degrees of freedom.  We consider the bi-Laplacian prior with
\begin{equation}\label{eq:prior_choice}
\Gamma_{\pr} = (\gamma I - \delta\Delta)^{-2} \revision{\text{ with }\gamma = 1 \text{ and }\delta = 8}{\text{ with }\gamma = 0.05 \text{ and }\delta = 10},
\end{equation}
where $I$ is the identity operator and $\Delta$ is the Laplacian operator on the given space.  In the discretized setting,  we consider the Ornstein-Uhlenbeck prior as defined in \eqref{eq:ornstein},   where its covariance matrix is parameterized with $\eta = 0.1$ and $\ell = 0.1$.  These parameters are heuristically chosen by empirical observations and prior knowledge of the given model following the literature \cite{kaltenbacher_2022,Pulkkinen_2014}. The implementation is done in Python with hIPPYlib library \cite{Villa_2021}. The system is solved using a conjugate gradient method implemented in the same library. \\
The code can be found at \url{https://github.com/hphuoctruong/fracPAT}.

\subsection{Influence of $\alpha$ and the choice of priors on reconstruction results}\label{sec:alpha}\text{}
In this first example,  we study the influence of $\alpha$ on the reconstruction results.  In the forward model \eqref{eq:wave_damped} as well as the adjoint model \eqref{eq:wave_equation_adjoint},  we consider $\alpha \in \{ 0.3,  0.8 \}$.  The damping coefficient in each case is $b = (-2c_0 r_0)/\cos (\pi (\alpha + 1)/2)$ \cite{Baker_2022},  where we choose $r_0 = 10^{-4}$. 
The intensity function is chosen of the form
\begin{equation}\label{eq:ref_intensity}
\iii_0 = \iii_0(t) = I_0\left[1 + \sin(\omega t)\right]
\end{equation}
 with $\omega = 100\pi$.
 %which is shown in Figure~\ref{eq:intensity}\todo{maybe skip this figure since it is not very telling}.
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.64\textwidth]{intensity.pdf}
%\caption{Reference intensity function $\iii_0$ and its derivative}
%\label{eq:intensity}
%\end{figure}
We consider Gaussian noise drawn from $\mathcal{N}(0,\sigma^2 I)$ with $\sigma^2 = 10^{-2}$.  

\noindent {\bf Influence of the choice of the differentiation order $\alpha$ in the damping.}  \revision{}{In order to illustrate the effect of $\alpha$ on the wave propagation, we display the state variable in both cases $\alpha \in \{ 0.3, 0.8 \}$ for $I_0 = 10^2$. Results are shown in Figure~\ref{fig:state_03} and Figure~\ref{fig:state_08}, respectively; while the wave forms look very similar, the different orders of magnitude clearly reflect the difference in the strength of attenuation.}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{state_variable_03.pdf}
	\caption{Snapshots of the state variable at $t \in \{ 0.01, 0.05, 0.1, 0.15, 0.2\}$ for $\alpha = 0.3$}
	\label{fig:state_03}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{state_variable_08.pdf}
	\caption{Snapshots of the state variable at $t \in \{ 0.01, 0.05, 0.1, 0.15, 0.2\}$ for $\alpha = 0.3$}
	\label{fig:state_08}
\end{figure}





\revision{}{We compare the MAP estimates given by \eqref{eq:map_estimator} using the bi-Laplacian prior}.  Reconstruction results for $\alpha \in \{0.3,  0.8\}$ together with the true solution are given in Figure \ref{fig:lowenergy}.  Here, one observes that with the weak damping $\alpha = 0.3$,  the ground truth is fairly well-reconstructed.  The result is smooth due to the smoothing property of the bi-Laplacian prior \eqref{eq:prior_choice}.  In the case of strong damping with $\alpha = 0.8$, the reconstruction quality is noticeably poorer, due to the significant loss of information by attenuation.  We numerically evaluate the reconstruction results for a realization of the Gaussian noise using the relative $L^2(\Omega)$ error $\norm{a - a_0}_{L^2(\Omega)}/\norm{a_0}_{L^2(\Omega)}$,  which is given in Table~\ref{tab:bilaplacian}.

In order to improve the reconstruction quality in the stronger damping case,  we increase the energy $I_0$ of the excitation function by a factor of four to $I_0 = 4\cdot 10^2$.  Reconstruction results in the setting with high energy are shown in Figure~\ref{fig:highenergy}.  Here,  one can see that there is an obvious improvement over the reconstructions in Figure~\ref{fig:lowenergy}.   The reconstruction errors in both cases are given in Table~\ref{tab:bilaplacian}.  In addition,  since only the temporal change $\iii'$,  rather than the values $\iii$ enter the model, it is obvious that improvements can be made by increasing the frequency of the excitation function.
We note that safety guidelines regarding the maximum light fluence or power limitations of the excitation laser must be closely monitored in practical situations, though, which is why we put a constraint on the magnitude of  $\iii'$.

%
\begin{figure}[h]
    \centering
        \includegraphics[width=0.32\textwidth]{u_init.pdf}
        \includegraphics[width=0.32\textwidth]{03_100_init_biLaplacian_new.pdf}
        \includegraphics[width=0.32\textwidth]{08_100_init_biLaplacian_new.pdf}
    \caption{Ground truth (left) and reconstruction results for $\alpha = 0.3$ (middle) and $\alpha = 0.8$ (right) with $I_0 = 10^2$ with the bi-Laplacian prior}
    \label{fig:lowenergy}
\end{figure}

\begin{figure}[h]
    \centering
        \includegraphics[width=0.32\textwidth]{u_init.pdf}
        \includegraphics[width=0.32\textwidth]{03_400_init_biLaplacian_new.pdf}
        \includegraphics[width=0.32\textwidth]{08_400_init_biLaplacian_new.pdf}
    \caption{Reconstruction results for $\alpha = 0.3$ (middle) and $\alpha = 0.8$ (right) with $I_0 = 4\cdot 10^2$ and  the bi-Laplacian prior}
    \label{fig:highenergy}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{l|cc}
\multicolumn{1}{c|}{} & \begin{tabular}[c]{@{}c@{}}Weak damping\\ $\alpha = 0.3$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Strong damping\\ $\alpha = 0.8$\end{tabular} \\ \hline
$I_ 0 = 10^2$				& $\revision{ 35.66 \%}{36.25 \%}$ 	& $\revision{ 58.19 \%}{64.00 \%} $                                                                    \\
$I_0 = 4 \cdot 10^2$   & $\revision{ 29.54 \%}{31.28 \%}$   & $\revision{49.90 \%}{53.09 \%}$                                                                   
\end{tabular}
\caption{Reconstruction errors with bi-Laplacian prior for different strengths of damping and different excitation amplitudes.}
\label{tab:bilaplacian}
\end{table}

\noindent {\bf Influence of the choice of priors.} Next, we investigate the selection of the prior distribution, acknowledging its substantial influence on the MAP estimates.  In this context, we compare the reconstruction results using the bi-Laplacian prior in the first example with those obtained using a Gaussian prior with an Ornstein-Uhlenbeck covariance matrix.  We study both strong and weak damping cases corresponding to $\alpha \in \{ 0.3,  0.8 \}$.  We choose the intensity function as in \eqref{eq:ref_intensity} with $I_0 = 10^2$.  With the same realization of noise as in the first example, a comparison of the reconstruction errors is given in Table~\ref{tab:bilaplacianvsornstein}.
\begin{table}[h!]
\centering
\begin{tabular}{l|cc}
\multicolumn{1}{c|}{}	 & Bi-Laplacian prior 											& Ornstein-Uhlenbeck prior \\ \hline
$\alpha = 0.3$				& $\revision{35.66 \%}{36.25 \%}$ 				  & $28.81\%$                \\
$\alpha = 0.8$				& $\revision{58.19 \%}{64.00 \%}$          	 & $51.94\%$               
\end{tabular}
\caption{Reconstruction error for different strengths of damping and different priors with $I_0 = 10^2$.}
\label{tab:bilaplacianvsornstein}
\end{table}
We observe that the MAP estimate using the Ornstein-Uhlenbeck prior performs notably better than the one using the bi-Laplacian prior, particularly in preserving the sharp edges of the ground truth. In contrast, the bi-Laplacian prior produces a smoother result, reflecting its natural tendency to smooth the reconstruction.  Nevertheless, in the strong damping case, the reconstruction quality in both scenarios is significantly poorer, primarily due to the substantial loss of energy as the wave travels through the medium.  For illustration,  we provide the MAP estimates in Figure~\ref{fig:ornsteinprior} with $I_0 = 10^2$ and $\alpha = 0.3$.
\begin{figure}[ht]
    \centering
        \includegraphics[width=0.32\textwidth]{u_init.pdf}
        \includegraphics[width=0.32\textwidth]{03_100_init_biLaplacian_new_2.pdf}
        \includegraphics[width=0.32\textwidth]{03_100_init_Ornstein_2.pdf}
    \caption{Reconstruction results with bi-Laplacian prior (middle) and Ornstein-Uhlenbeck prior (right) with $I_0 = 10^2$ and $\alpha = 0.3$ }
    \label{fig:ornsteinprior}
\end{figure}

\subsection{Optimization of laser intensity function}
We next study the problem of optimizing the laser intensity function which is considered as a design variable.  Here,  in order to focus on choosing the intensity function,  we remain with the weak damping case $\alpha = 0.3$.  Following Section~\ref{sec:computation_functional},  the intensity function is assumed to be band-limited.  To obtain this,  we consider a signal that has finite number of $K$ active frequencies,  namely
\begin{equation}\label{eq:i_form}
\iii = \iii(t;I,  \coeffi_1,\ldots,\coeffi_K) = I\left[1 +
\sum_{k=1}^K \coeffi_k\sin(k \omega t)\right],
\end{equation}
where $\omega_k,  k = 1,\ldots, K$ are fixed and $I,  \bo{\coeffi}= (\coeffi_1,  \ldots,  \coeffi_K)$ are variables. 
The optimal laser intensity that we are looking for should in addition fulfill the following conditions:
\begin{itemize}
\item[$\bullet$] $\iii \ge 0$,  in view of the fact that only nonnegative laser intensities make sense physically.  
\item[$\bullet$] $\iii$ has bounded $H_1$ norm to satisfy bounds on the energy. Such a constraint of the $H^1-$norm and thus on the high frequency content of the signal also make sense in view of the fact that higher frequencies undergo more significant attenuation while propagating through the medium.
\end{itemize}
Hence,  we consider the set
\begin{equation}\label{eq:admissible_set}
\mathcal{D}:= \left\{ \iii \in H^1(0,T): \iii \text{ is of the form }\eqref{eq:i_form},  |\bo{\coeffi}|_1 \le 1,  \norm{\iii}_{H^1(0,1)} \le M := 4\norm{\iii_0} \right\},
\end{equation}
where the constraint $|\bo{\coeffi}|_1 \le 1$ guarantees the positivity of $\iii$ and the latter ensures that the norm of 
$\iii$ is sufficiently bounded yet allows room for variations in the optimization process.  Note that $\mathcal{D}$ is a (weakly) compact subset of $H^1(0,T)$.

Turning to the optimality criterion,  we consider the approximated $A$-optimality cost functional $\varphi_N$ via projections given in ~\eqref{eq:A_optimal_projected}.  We choose the projections onto finite-dimensional subspaces spanned by the eigenvectors of the prior covariance operators of both bi-Laplacian prior and Ornstein-Uhlenbeck prior.  The decays of the eigenvalues in both cases are illustrated in Figure~\ref{fig:decay}.

\begin{figure}[h]
\includegraphics[width=0.48\textwidth]{eigenvalues_biLaplacian_new.pdf}
\includegraphics[width=0.48\textwidth]{eigenvalues_Ornstein_new.pdf}
\caption{Decay of eigenvalues of $\bo{\Gamma}_{\pr}$ for bi-Laplacian prior (left) and Ornstein-Uhlenbeck-prior (right)}
\label{fig:decay}
\end{figure}
In the first case,  observing that the decay of eigenvalues  is sufficiently fast,  we consider the projection onto $X_N$, spanned by the first $N$ eigenfunctions, with $N = 160$.  Since $\iii$ in this setting is parametrized by $I, \bo{\coeffi}$ as in \eqref{eq:admissible_set},  we solve the optimization problem
\begin{equation}
\va{ &\Psi_N(I,  \bo{\coeffi}) = \varphi_N(\iii) = \tr_{\bo{M}} (\bo{\Gamma}^N_{\post}(\iii)) \to \min, \\
&\text{ subject to } \iii \in \mathcal{D}.}
\end{equation}
In the optimization process,  we use the initial guess $(I_0,  \bo{\coeffi}_0)$ with $I_0 = 10^{2}$ and $\bo{\coeffi}_0 = (1,0,0,\ldots)$,  which corresponds to the reference intensity function $\iii_0$ used in Section~\ref{sec:alpha}. 
The number of frequencies was chosen as $K=5$; a larger choice did not yield any significant changes. We note that $\Psi_N$ is monotone in $I$ and therefore $\Psi_N(I,  \bo{\coeffi}) \ge \Psi(4I_0,  \bo{\coeffi})$ due to the constraint $\norm{\iii}_{H^1(0,T)} \le 4 \norm{\iii_0}_{H^1(0,1)}$,  which reduces the problem to optimizing over $\bo{\coeffi}$.  The optimization process yields the coefficients $(I_{\text{opt}},  \bo{\coeffi}_{\text{opt}})$ with $I_{\text{opt}} = 4 \cdot 10^2$ and $\bo{\coeffi}_{\text{opt}} = \revision{}{(0.4238,  0.2196,  0.1487,  0.1136,  0.0942)}$,  from which the optimal intensity function $\iii_{\text{opt}}$ results according to \eqref{eq:i_form}.  Values of the $A$-optimality cost functional for $\iii_0$ and $\iii_{\text{opt}}$ are shown in  Table~\ref{tab:optimal_values}, where it is evident that the obtained solutions significantly improve the approximated average reconstruction results.  We note that due to the nonconvex nature of the cost functional,  the optimal solution $\iii_{\text{opt}}$ is only a local solution.  In the case of the Ornstein-Uhlenbeck prior, although the decay is not sufficiently rapid, we still project onto the space spanned by the first $N=160$ eigenfunctions to render the minimization problem computationally tractable.  We again obtain an optimal solution $(I_{\text{opt}}, \bo{\coeffi}_{\text{opt}})$ with $I_{\text{opt}} = 4 \cdot 10^2$ and $\bo{\coeffi}_{\text{opt}} = (0.4229, 0.2202, 0.1495,  0.1136,  0.0937)$. Results are shown in Table~\ref{tab:optimal_values},  where one can also see that this also significantly improves on $A$-optimality.  

\revision{}{To demonstrate the effect of the initial and optimal intensity functions on wave propagation, we plot snapshots of the wave field resulting from the reconstructed absorption density function $a$ at different time steps. Here, we again select the time instances $t \in \{ 0.01, 0.05, 0.1, 0.15, 0.2\}$. Results are shown in Figure~\ref{fig:state_i0} and Figure~\ref{fig:state_iopt}.}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{state_variable_i0.pdf}
	\caption{Snapshots of the state variable at $t \in \{ 0.01, 0.05, 0.1, 0.15, 0.2\}$ for $a$ reconstructed with $i = i_0$}
	\label{fig:state_i0}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{state_variable_iopt.pdf}
	\caption{Snapshots of the state variable at $t \in \{ 0.01, 0.05, 0.1, 0.15, 0.2\}$ for $a$ reconstructed with $i = i_{\text{opt}}$}
	\label{fig:state_iopt}
\end{figure}

Finally, to numerically verify the improvement, we consider the reconstruction problem with the realization of noise considered in Section~\ref{sec:alpha} and compare reconstruction results using $\iii_0$ and $\iii_{\text{opt}}$.  The reconstruction results, summarized in Table~\ref{tab:optimal_values}, demonstrate a significant enhancement in accuracy. Specifically, in the bi-Laplacian case, the reconstruction error is reduced by $\revision{9.61\%}{9.00\%}$, indicating a notable performance gain. In the Ornstein-Uhlenbeck case, despite a smaller improvement, the reconstruction error still decreases by $6.55\%$.  Both show the relative improvement of $\revision{26.62\%}{24.83\%}$ and $22.74\%$,  respectively. 

Notably, the maximum frequency (under the given constraints) excitation function $\iii$ determined by the coefficients $(0,0,0,0,0.2)$ is not optimal.  Reconstruction errors with this choice are $\revision{28.52\%}{29.76\%}$ and $23.68\%$,  respectively. 
This shows that choosing a more sophisticated intensity function by means of mathematical optimization indeed pays off.

\begin{table}[h]
\begin{tabular}{c|cc|cc}
                                                                                & \multicolumn{2}{c|}{Bi-Laplacian prior}                            & \multicolumn{2}{c}{Ornstein-Uhlenbeck prior}                       \\ \cline{2-5} 
\multicolumn{1}{l|}{}                                                           & \multicolumn{1}{c|}{Relative error} & $\varphi_N(\iii)$ & \multicolumn{1}{c|}{Relative error} & $\varphi_N(\iii)$ \\ \hline
\begin{tabular}[c]{@{}c@{}}Initial guess\\ $I_0 = 10^2,  \bo{\coeffi}_0$\end{tabular}            
& \multicolumn{1}{c|}{$\revision{35.66 \%}{36.25 \%}$}              & $\revision{0.353}{0.193}$              
& \multicolumn{1}{c|}{$28.81\%$}              & $2.428$              \\ \hline
\begin{tabular}[c]{@{}c@{}}Optimal solution\\ $I_{\text{opt}} = 4\cdot 10^2,  \bo{\coeffi}_{\text{opt}}$\end{tabular} 
& \multicolumn{1}{c|}{$\revision{\bld{26.05 \%}}{\bld{27.25 \%}}$}             & $\revision{\bld{0.101}}{\bld{0.063}}$              
& \multicolumn{1}{c|}{$\bld{22.26\%}$}              & $\bld{0.278}$             
\end{tabular}
\caption{Reconstruction errors with initial and optimal intensity functions for $\alpha = 0.3$}
\label{tab:optimal_values}
\end{table}






